Bag of Tricks for Effective Language Model Pretraining and Downstream Adaptation: A Case Study on GLUE

This technical report briefly describes our JDExplore d-team's submission Vega v1 on the General Language Understanding Evaluation (GLUE) leaderboard, where GLUE is a collection of nine natural language understanding tasks, including question answering, linguistic acceptability, sentiment analysis, text similarity, paraphrase detection, and natural language inference. [Method] We investigate several effective strategies and choose their best combination setting as the training recipes. As for model structure, we employ the vanilla Transformer with disentangled attention as the basic block encoder. For self-supervised training, we employ the representative denoising objective (i.e., replaced token detection) in phase 1 and combine the contrastive objective (i.e., sentence embedding contrastive learning) with it in phase 2. During fine-tuning, several advanced techniques such as transductive fine-tuning, self-calibrated fine-tuning, and adversarial fine-tuning are adopted. [Results] According to our submission record (Jan. 2022), with our optimized pretraining and fine-tuning strategies, our 1.3 billion model sets new state-of-the-art on 4/9 tasks, achieving the best average score of 91.3. Encouragingly, our Vega v1 is the first to exceed powerful human performance on the two challenging tasks, i.e., SST-2 and WNLI. We believe our empirically successful recipe with a bag of tricks could shed new light on developing efficient discriminative large language models.

==> [TechReport2022] Vega-V1/all_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{\label{tab:ranking} \textbf{Ranking of our submission in terms of average score} in the GLUE leaderboard (\url{https://gluebenchmark.com/leaderboard}) on January 1, 2022.}
\scalebox{0.7}{
\begin{tabular}{clcccccccccccccc}
\toprule
 & \multicolumn{1}{c}{} & CoLA & SST-2 & \multicolumn{2}{c}{MRPC} & \multicolumn{2}{c}{STS-B} & \multicolumn{2}{c}{QQP} & \multicolumn{2}{c}{MNLI} & QNLI & RTE & WNLI &  \\ \cmidrule{3-15}
\multirow{-2}{*}{Rank} & \multirow{-2}{*}{Models} & \textit{Mcc.} & \textit{Acc.} & \textit{F1} & \textit{Acc.} & \textit{Pcor.} & \textit{Scor.} & F1 & Acc. & \textit{m.} & \textit{mm.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \multirow{-2}{*}{Score} \\ \midrule \midrule
1 & Vega v1 & 73.8 & 97.9 & 94.5 & 92.6 & 93.5 & 93.1 & 76.7 & 91.1 & 92.1 & 91.9 & 96.7 & 92.4 & 97.9 & 91.3 \\
2 & TuringNLR v5 & 72.6 & 97.6 & 93.8 & 91.7 & 93.7 & 93.3 & 76.4 & 91.1 & 92.6 & 92.4 & 97.9 & 94.1 & 95.9 & 91.2 \\
3 & ERNIE & 75.5 & 97.8 & 93.9 & 91.8 & 93.0 & 92.6 & 75.2 & 90.9 & 92.3 & 91.7 & 97.3 & 92.6 & 95.9 & 91.1 \\
4 & StructBERT + CLEVER & 75.3 & 97.7 & 93.9 & 91.9 & 93.5 & 93.1 & 75.6 & 90.8 & 91.7 & 91.5 & 97.4 & 92.5 & 95.2 & 91.0 \\
5 & DeBERT + CLEVER & 74.2 & 97.5 & 93.3 & 91.0 & 93.4 & 93.1 & 76.4 & 90.9 & 92.1 & 91.7 & 96.7 & 93.1 & 96.6 & 91.0 \\
6 & DeBERTa / TuringNLRv4 & 71.5 & 97.5 & 94.0 & 92.0 & 92.9 & 92.6 & 76.2 & 90.8 & 91.9 & 91.6 & 99.2 & 93.2 & 94.5 & 90.8 \\
7 & MacALBERT + DKM & 74.8 & 97.0 & 94.5 & 92.6 & 92.8 & 92.6 & 74.7 & 90.6 & 91.3 & 91.1 & 97.8 & 92.0 & 94.5 & 90.7 \\
8 & ALBERT + DAAF + NAS & 73.5 & 97.2 & 94.0 & 92.0 & 93.0 & 92.4 & 76.1 & 91.0 & 91.6 & 91.3 & 97.5 & 91.7 & 94.5 & 90.6 \\
9 & T5 & 71.6 & 97.5 & 92.8 & 90.4 & 93.1 & 92.8 & 75.1 & 90.6 & 92.2 & 91.9 & 96.9 & 92.8 & 94.5 & 90.3 \\
10 & MT-DNN-SMART & 69.5 & 97.5 & 93.7 & 91.6 & 92.9 & 92.5 & 73.9 & 90.2 & 91.0 & 90.8 & 99.2 & 89.7 & 94.5 & 89.9 \\
11 & NEZHA-Large & 71.7 & 97.3 & 93.3 & 91.0 & 92.4 & 91.9 & 75.2 & 90.7 & 91.5 & 91.3 & 96.2 & 90.3 & 94.5 & 89.9 \\
12 & Funnel-Transformer & 70.5 & 97.5 & 93.4 & 91.2 & 92.6 & 92.3 & 75.4 & 90.7 & 91.4 & 91.1 & 95.8 & 90.0 & 94.5 & 89.7 \\
13 & ELECTRA-Large-large & 71.7 & 97.1 & 93.1 & 90.7 & 92.9 & 92.5 & 75.6 & 90.8 & 91.3 & 90.8 & 95.8 & 89.8 & 91.8 & 89.4 \\
14 & DropAK-ELECTRA-large & 70.4 & 95.8 & 92.6 & 90.1 & 91.2 & 91.1 & 75.1 & 90.5 & 91.1 & 90.9 & 93.8 & 90.1 & 91.8 & 88.7 \\
15 & FreeLB-RoBERTa & 68.0 & 96.8 & 93.1 & 90.8 & 92.3 & 92.1 & 74.8 & 90.3 & 91.1 & 90.7 & 95.6 & 88.7 & 89.0 & 88.4 \\
16 & HIRE-RoBERTa & 68.6 & 97.1 & 93.0 & 90.7 & 92.4 & 92.0 & 74.3 & 90.2 & 90.7 & 90.4 & 95.5 & 87.9 & 89.0 & 88.3 \\
17 & ELECTRA-large-M & 69.3 & 95.8 & 92.2 & 89.6 & 91.2 & 91.1 & 75.1 & 90.5 & 91.1 & 90.9 & 93.8 & 87.9 & 91.8 & 88.3 \\
18 & RoBERTa & 67.8 & 96.7 & 92.3 & 89.8 & 92.2 & 91.9 & 74.3 & 90.2 & 90.8 & 90.2 & 95.4 & 88.2 & 89.0 & 88.1 \\
19 & MT-DNN-ensemble & 68.4 & 96.5 & 92.7 & 90.3 & 91.1 & 90.7 & 73.7 & 89.9 & 87.9 & 87.4 & 96.0 & 86.3 & 89.0 & 87.6 \\
20 & GLUE Human Baselines & 66.4 & 97.8 & 86.3 & 80.8 & 92.7 & 92.6 & 59.5 & 80.4 & 92.0 & 92.8 & 91.2 & 93.6 & 95.9 & 87.1 \\
\bottomrule
\end{tabular}
}
\label{tab:allrank}
\end{table*}

==> [TechReport2022] Vega-V1/main_results.tex <==
\begin{table*}[ht]
\caption{\textbf{Results obtained on the GLUE test sets}, which are scored by the GLUE evaluation server. We obtained the results from \url{https://gluebenchmark.com/leaderboard} on January 1, 2022. The best results (except those of human baselines) are shown in bold.}
\scalebox{0.73}{
\centering
\begin{tabular}{lcccccccccccccc}
\toprule
\multicolumn{1}{c}{} & CoLA & SST-2 & \multicolumn{2}{c}{MRPC} & \multicolumn{2}{c}{STS-B} & \multicolumn{2}{c}{QQP} & \multicolumn{2}{c}{MNLI} & QNLI & RTE & WNLI &  \\ \cmidrule{2-14}
\multirow{-2}{*}{\textbf{Models}} & \textit{Mcc.} & \textit{Acc.} & \textit{F1} & \textit{Acc.} & \textit{Pcor.} & \textit{Scor.} & \textit{F1} & \textit{Acc.} & \textit{m.} & \textit{mm.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \multirow{-2}{*}{Score} \\ \midrule \midrule
\textbf{GLUE Human Baselines} & 66.4 & 97.8 & 86.3 & 80.8 & 92.7 & 92.6 & 59.5 & 80.4 & 92.0 & 92.8 & 91.2 & 93.6 & 95.9 & 87.1 \\ \hdashline
\textbf{T5} & 71.6 & 97.5 & 92.8 & 90.4 & 93.1 & 92.8 & 75.1 & 90.6 & 92.2 & 91.9 & 96.9 & 92.8 & 94.5 & 90.3 \\
\textbf{ALBERT + DAAF + NAS} & 73.5 & 97.2 & 94.0 & 92.0 & 93.0 & 92.4 & 76.1 & 91.0 & 91.6 & 91.3 & 97.5 & 91.7 & 94.5 & 90.6 \\
\textbf{MacALBERT + DKM} & 74.8 & 97.0 & \textbf{94.5} & \textbf{92.6} & 92.8 & 92.6 & 74.7 & 90.6 & 91.3 & 91.1 & 97.8 & 92.0 & 94.5 & 90.7 \\
\textbf{DeBERTa / TuringNLRv4} & 71.5 & 97.5 & 94.0 & 92.0 & 92.9 & 92.6 & 76.2 & 90.8 & 91.9 & 91.6 & \textbf{99.2} & 93.2 & 94.5 & 90.8 \\
\textbf{DeBERT + CLEVER} & 74.2 & 97.5 & 93.3 & 91.0 & 93.4 & 93.1 & 76.4 & 90.9 & 92.1 & 91.7 & 96.7 & 93.1 & 96.6 & 91.0 \\
\textbf{StructBERT + CLEVER} & 75.3 & 97.7 & 93.9 & 91.9 & 93.5 & 93.1 & 75.6 & 90.8 & 91.7 & 91.5 & 97.4 & 92.5 & 95.2 & 91.0 \\
\textbf{ERNIE} & \textbf{75.5} & 97.8 & 93.9 & 91.8 & 93.0 & 92.6 & 75.2 & 90.9 & 92.3 & 91.7 & 97.3 & 92.6 & 95.9 & 91.1 \\
\textbf{TuringNLR v5} & 72.6 & 97.6 & 93.8 & 91.7 & \textbf{93.7} & \textbf{93.3} & 76.4 & 91.1 & \textbf{92.6} & \textbf{92.4} & 97.9 & \textbf{94.1} & 95.9 & 91.2 \\ \midrule
\textbf{Vega v1 (Ours)} & 73.8 & \textbf{97.9} & \textbf{94.5} & \textbf{92.6} & 93.5 & 93.1 & \textbf{76.7} & \textbf{91.1} & 92.1 & 91.9 & 96.7 & 92.4 & \textbf{97.9} & \textbf{91.3} \\
\bottomrule
\end{tabular}
}
\label{table_main}
\end{table*}

==> [TechReport2022] Vega-V1/task_descriptions.tex <==
\begin{table*}[t]
\centering \small
\caption{\textbf{Task descriptions and statistics}. All tasks are single sentence or sentence pair classification, except STS-B, which is a regression task. MNLI has three classes; all other classification tasks have two. Test sets shown in bold use labels that have never been made public in any form.
}
\begin{tabular}{lrrlll}
 \toprule
\textbf{Corpus} & \textbf{$|$Train$|$} & \textbf{$|$Test$|$} & \textbf{Task} & \textbf{Metrics} & \textbf{Domain} \\
\midrule
\multicolumn{6}{c}{Single-Sentence Tasks}\\
\midrule
CoLA & 8.5k & \textbf{1k} & acceptability & Matthews corr.& misc. \\ % SB: Changed from 'linguistics literature'. That could be misleading, as few of the sentences are actually in the style of academic writing, and many are found in the wild.
SST-2 & 67k & 1.8k & sentiment & acc. & movie reviews \\
\midrule
\multicolumn{6}{c}{Similarity and Paraphrase Tasks}\\
\midrule
MRPC & 3.7k & 1.7k & paraphrase & acc./F1 & news \\
STS-B & 7k & 1.4k & sentence similarity & Pearson/Spearman corr. & misc. \\
QQP & 364k & \textbf{391k} & paraphrase & acc./F1 & social QA questions \\
\midrule
\multicolumn{6}{c}{Inference Tasks} \\
\midrule
MNLI & 393k & \textbf{20k} & NLI & matched acc./mismatched acc. & misc. \\
QNLI & 108k & 5.7k & QA/NLI & acc. & Wikipedia \\
RTE & 2.5k & 3k & NLI & acc. & misc. \\
WNLI & 634 & \textbf{146} & coreference/NLI & acc. & fiction books \\
\bottomrule
\end{tabular}
\label{tab:tasks}
\end{table*}
